VBR: Version Based Reclamation

Safe lock-free memory reclamation is a difficult problem. Existing solutions follow three basic methods (or their combinations): epoch based reclamation, hazard pointers, and optimistic reclamation. Epoch-based methods are fast, but do not guarantee lock-freedom. Hazard pointer solutions are lock-free but typically do not provide high performance. Optimistic methods are lock-free and fast, but previous optimistic methods did not go all the way. While reads were executed optimistically, writes were protected by hazard pointers. In this work we present a new reclamation scheme called version based reclamation (VBR), which provides a full optimistic solution to lock-free memory reclamation, obtaining lock-freedom and high efficiency. Speculative execution is known as a fundamental tool for improving performance in various areas of computer science, and indeed evaluation with a lock-free linked-list, hash-table and skip-list shows that VBR outperforms state-of-the-art existing solutions.

==> conclusions.tex <==
\section{Conclusions} \label{sec-conclusions}

This paper presents VBR, the first fully optimistic safe memory reclamation scheme, allowing threads to access reclaimed objects for both reads and writes. VBR is fast, widely applicable and lock-free.
The versioning mechanism guarantees that stale values are always ignored and writes to reclaimed objects always fail.
The fully speculative execution yields a drastic reduction in the reclamation overheads compared to other safe reclamation algorithms. Measurements demonstrate that VBR outperforms state-of-the-art safe memory reclamation algorithms for several data-structures and varying workloads.



==> optimizations.tex <==
\section{Optimizations} \label{sec-optimizations}
